An Optimal Algorithm for Finding Champions in Tournament Graphs

A tournament graph is a complete directed graph, which can be used to model a round-robin tournament between $n$ players. In this paper, we address the problem of finding a champion of the tournament, also known as Copeland winner, which is a player that wins the highest number of matches. In detail, we aim to investigate algorithms that find the champion by playing a low number of matches. Solving this problem allows us to speed up several Information Retrieval and Recommender System applications, including question answering, conversational search, etc. Indeed, these applications often search for the champion inducing a round-robin tournament among the players by employing a machine learning model to estimate who wins each pairwise comparison. Our contribution, thus, allows finding the champion by performing a low number of model inferences. We prove that any deterministic or randomized algorithm finding a champion with constant success probability requires $\Omega(\ell n)$ comparisons, where $\ell$ is the number of matches lost by the champion. We then present an asymptotically-optimal deterministic algorithm matching this lower bound without knowing $\ell$, and we extend our analysis to three variants of the problem. Lastly, we conduct a comprehensive experimental assessment of the proposed algorithms on a question answering task on public data. Results show that our proposed algorithms speed up the retrieval of the champion up to $13\times$ with respect to the state-of-the-art algorithm that perform the full tournament.

==> sections/1-introduction-backup.tex <==
% !TEX root = ../paper.tex
% !TeX spellcheck = en_US

\section{Introduction}
\label{bf:sec:intro}

The identification of the most relevant results from a pool of candidates is known as the \emph{ranking} task and it is crucial in many Information Retrieval and Recommender System applications including ad-hoc search~\cite{baeza1999modern}, conversational search~\cite{DBLP:conf/cikm/Maarek18}, question answering~\cite{DBLP:journals/tois/HerlockerKTR04}, machine translation, etc.
A classic example of a ranking task is ad-hoc search, where a user submits a textual query to a search engine, e.g., Google, and the system returns the $k$---tipically $10$---results with highest relevance with respect to the query.
A more recent example in that line are conversational assistants.
These devices, such as Siri, Google Assistant, and Alexa, are becoming very popular nowadays.
They work by exploiting a new way of interaction with the user, where the latter interacts by asking a question and the former provides her the most relevant answer to the question.
Conversational assistants introduce a \emph{paradigm shift} in information retrieval as they change the way users submit their information needs to the information retrieval system, i.e., using spoken words and not textual queries.
Moreover, due to the fact that the new paradigm employs a conversation as a mean of interaction, only one result is provided to the user as an answer to her question. As a consequence, the precision of the information retrieval system that identifies the only answer to return is now of paramount importance to build an effective conversational system.
State-of-the-art solutions for ranking leverage ad-hoc machine learning techniques, known as Learning-to-Rank~\cite{DBLP:journals/ftir/Liu09}, to score the candidate results and select the top-$1$ achieving the highest relevance score.
The retrieval of the most relevant result can be addressed in two different ways:
\textit{i}) by exploiting state-of-the-art Learning-to-Rank techniques such as \lmart~\cite{DBLP:journals/ir/WuBSG10}, which are based on univariate scoring functions that individually score one candidate result at a time, to select the candidate achieving the highest score;
\textit{ii}) by employing pairwise Learning-to-Rank techniques such as \dbert{} \cite{DBLP:journals/corr/abs-1901-04085}, which are based on bivariate scoring functions that score a pair of candidate results at a time, e.g., a binary judgment stating which of the results is more relevant, to select the candidate achieving the highest sum of pairwise scores of an all-vs-all tournament.
While the former approach exploits only the information of a single result at a time for computing the ranking score, the latter approach is potentially more powerful because it exploits the information of two candidates at a time for computing the outcome of the tournament.
However, the latter approach is more expensive than the former one as it performs a quadratic number of comparisons to score all pairs of candidate results, thus making pairwise approaches unappealing in scenarios with tight time constraints.

In this article, we focus on pairwise techniques by investigating algorithmic approaches that allow to reduce the number of comparisons performed to score candidate results. We contribute to this goal by modeling the problem of efficiently retrieving the most relevant result from a list of candidate results as the task of finding a champion, also known as the \textit{Copeland winner}~\cite{GS:copeland1951reasonable}, i.e., the player that wins the highest number of matches, of a round-robin tournament~\cite{GS:reid2013tournaments}. We model the round-robin tournament as an acyclic graph, where edges connecting vertices represent a match played between the two vertices and the direction of the edge models who wins between the two players. We define the champion as the player, i.e., one vertex of the tournament graph, that wins the highest number of matches in the tournament.

\subsubsection*{Our Contribution}
We rely on the tournament graph to investigate efficient algorithms that allow to reduce the number of comparisons performed in the tournament. The novel and unpublished contributions of this article are the following:
\begin{itemize}[leftmargin=*]
	\item we introduce an asymptotically-optimal deterministic algorithm that finds the champion by employing $\Theta(\ell n)$ vertex comparisons, where $\ell$ is the minimum number of matches lost by any player. Moreover, we prove that $\Omega(\ell n)$ comparisons are necessary, even for randomized algorithms, to obtain a correct answer with any constant probability. It is worth to notice that we match a randomized lower bound with a deterministic algorithm, showing that randomization does not give any advantage on this problem.
	\item We extend our result to three strictly related problems. First, we show how to retrieve all top-$k$ players in time $O(\ell_k n)$, where $\ell_k$ is the number of matches lost by the $k$-th best player. Second, we consider a model of computation in which we are allowed to play a batch of $B$ matches in parallel, and we design an algorithm that achieves optimal speedup with respect to the sequential version. Third, we suppose that playing a match does not return a binary result, but a distribution over the outcomes, i.e., a pair of complementary probabilities. In this setting, we define the champion as the player that minimizes the expected number of matches lost and we introduce an algorithm to find all champions in time $\Theta(\ell n)$, where $\ell$ is the expected number of matches lost by the champion.
	\item We provide a comprehensive experimental assessment of the proposed algorithms. We evaluate their performance in terms of running time and number of comparisons, which are then compared with respect to a baseline that perform all the possible pairwise comparisons between players. We focus our attention on the execution of the three-stage ranking architecture introduced by Nogueira \etal{}~\cite{DBLP:journals/corr/abs-1910-14424}. Results show that our proposed algorithms achieve a remarkable speedup of up to $13\times$ with respect to methods that work by playing the full tournament.
\end{itemize}

The rest of the article is structured as follows: Section~\ref{bf:sec:related} discusses the related work, while Section~\ref{bf:sec:problem_definition} defines the problem. Section~\ref{bf:sec:complexity} provides a detailed analysis of the problem complexity and Section~\ref{bf:sec:algorithm} presents an efficient algorithm to solve it. Moreover, Section~\ref{bf:sec:generalizations} discusses two variants of that algorithm that solve two extensions of the original problem. Finally, Section~\ref{bf:sec:experiments} presents a comprehensive analysis of proposed algorithms in a information retrieval (ad-hoc search) scenario, and Section~\ref{bf:sec:summary} concludes the work.


==> sections/1-introduction.tex <==
% !TEX root = ../paper.tex
% !TeX spellcheck = en_US

\section{Introduction}
\label{bf:sec:intro}
A \emph{tournament graph} is a complete directed graph $T = \left(V, E \right)$.
This graph can be used to model a round-robin tournament between $n$ players, where each player plays a match with any other player.
The orientation of an arc in $E$ tells the winner of the match, i.e., we have the arc $(u, v) \in E$ iff $u$ beats $v$ in their match.

We address the problem of finding a champion of the tournament, also known as \textit{Copeland winner}~\cite{GS:copeland1951reasonable}, which is a vertex in $V$ with the maximum out-degree, i.e., a player that wins the highest number of matches.
Our goal is to find a champion by minimizing the number of {\em arc lookup}s, i.e., the number of played matches.
Note that a tournament graph may have more than one champion.
In this case, we aim at finding any of them, even if all the algorithms are able to find all of them without increasing the complexity.

If the tournament is transitive (i.e., if $u$ wins against $v$ and $v$ wins against $w$, then $u$ wins against $w$), we can trivially identifying the (unique) champion with $\Theta(n)$ arc lookups.
Indeed, the champion is the only vertex that wins all its matches and, thus, we can perform a \textit{knock-out tournament} where the loser of any match is immediately eliminated.
However, finding the champion of general tournament graphs requires $\Omega(n^2)$ arc lookups \cite{DBLP:journals/corr/GutinMR18}, and thus, there is nothing better to do than play all the matches.
This means that the structure of the underlying tournament graph heavily impacts the complexity of the problem.

\In this article, we investigate efficient algorithms requiring a number of arc lookups which depends on the number of matches lost by the champion of the tournament. Later on, we will see that this parametrization is motivated by many applications in Information Retrieval and Recommender Systems, where we expect that a champion, e.g., the best item in a set, loses only few matches.
%\lb{Ho usato grassetto + noindent preché ho visto che lo aveva fatto FM piú sotto. Poi mi é venuto il sospetto che non sia accettato dall'editore, a volte preferiscono che si usino solo i comandi del template. Sicuramente voi che avete piú esperienza questo lo sapete meglio.}
%\lb{\noindent \textbf{Tournaments as imprecise comparisons}.
These applications often relies on machine learning (ML) algorithms that given two items return which of the two is \emph{better}, according to an application-specific definition of quality.
The set of all these comparisons induces a---possibly non-transitive---tournament graph over all items.
Consider the task of retrieving the \emph{best item}, i.e., the champion of the tournament, this can be meaningfully defined as the Copeland winner.
Moreover, an effective ML algorithm is expected to make few mistakes while comparing the champion.
This suggests that we should parameterize the complexity of finding the champion with respect to the number of comparisons lost by the champion.

\medskip
\noindent \textbf{Our Contributions}. The novel contributions of this article are the following:

\rt{
[IN SOSTITUZIONE DEL PEZZO GIALLO DI ROSS]
In this article, we investigate efficient algorithms requiring a number of arc lookups which depends on the number of matches lost by the champion of the tournament.
The problem we are facing has an interesting application in Information Retrieval, in particular in the task of identifying the most relevant result from a set of candidates.
Some effective techniques address this task by using pairwise ranking models, similar to machine learning classifiers, that compare a pair of candidate results at a time and select the candidate winning the highest number or pairwise comparisons of the all-vs-all tournament between the results\cite{GS:ai2019learning,DBLP:journals/corr/abs-1901-04085}.
In this setting, we expect that a champion loses only few matches.
For this reason, in this article, we look for efficient algorithmic solutions to find the tournament champion by performing the minimum number of ``classifications'' needed to solve this problem.
}

%\ross{In this article, we investigate efficient algorithms requiring a number of arc lookups which depends on the number of matches lost by the champion of the tournament. Later on, we will see that this parametrization is motivated by applications in Information Retrieval and Machine Learning where we expect that a champion (e.g., the best item in a set) loses only few matches.}

%\lb{Ho usato grassetto + noindent preché ho visto che lo aveva fatto FM piú sotto. Poi mi é venuto il sospetto che non sia accettato dall'editore, a volte preferiscono che si usino solo i comandi del template. Sicuramente voi che avete piú esperienza questo lo sapete meglio.}

\lb{\noindent \textbf{Tournaments as imprecise comparisons}.
Suppose that we have a ML algorithm that given two items returns which of the two is \emph{better}, the set of all these comparisons induces a (possibly non-transitive) tournament graph over all items.
Consider the task of retrieving the \emph{best item}, this can be meaningfully defined as the Copeland winner. Moreover, a well-behaved ML algorithm is expected to make few mistakes while comparing the best item. This suggests that we should parameterize the complexity of finding the champion with respect to the number of comparisons lost by the best item.}

\noindent \textbf{Our Contributions}. In detail, the \revrm{novel} contributions of this article are the following:
\begin{itemize}[leftmargin=*]
	\item we introduce an asymptotically-optimal deterministic algorithm that finds the champion by employing $O(\ell n)$ vertex comparisons, where $\ell$ is the minimum number of matches lost by any player. Moreover, we prove that $\Omega(\ell n)$ comparisons are necessary, even for randomized algorithms, to obtain a correct answer with any constant probability. It is worth to notice that we match a randomized lower bound with a deterministic algorithm, showing that randomization does not give any advantage on this problem.
	\item We extend our result to three strictly related problems. First, we show how to retrieve all top-$k$ players in time $O(\ell_k n)$, where $\ell_k$ is the number of matches lost by the $k$-th best player. Second, we consider a model of computation in which we are allowed to play a batch of $B$ matches in parallel, and we design an algorithm that achieves optimal speedup with respect to the sequential version. Third, we suppose that playing a match does not return a binary result, but a distribution over the outcomes, i.e., a pair of complementary probabilities. In this setting, we define the champion as the player that minimizes the expected number of matches lost and we introduce an algorithm to find all champions in time $\Theta(\ell n)$, where $\ell$ is the expected number of matches lost by the champion.
	\item We provide a comprehensive experimental assessment of the proposed algorithms. We evaluate their performance in terms of running time and number of comparisons against a baseline that perform all the possible pairwise comparisons between players. We focus our attention on a Question Answering task that asks to find the most relevant textual answer to a given question provided by a user~\cite{DBLP:journals/corr/abs-1910-14424}. Results show that our proposed algorithms allow to speed up the identification of the correct answer of up to $13\times$ with respect to methods that play the full tournament.
\end{itemize}

\noindent \textbf{Motivation}.
Such an investigation is motivated by many application scenarios involving efficiently selecting one item from a set of candidate items.
An example application scenario deals with the identification of the most relevant result from a pool of candidates.
This task is crucial in many Information Retrieval and Recommender System applications including ad-hoc search~\cite{baeza1999modern}, conversational search~\cite{DBLP:conf/cikm/Maarek18}, question answering~\cite{DBLP:journals/tois/HerlockerKTR04}, etc.
A recent example in this line are conversational assistants.
These devices, such as Siri, Google Assistant, and Alexa, are becoming very popular nowadays.
They work by exploiting a new way of interaction with the user, where the latter interacts by asking a question and the former provides her the answer with highest relevance with respect to the question.
Conversational assistants introduce a \emph{paradigm shift} in information retrieval as they change the way users submit their information needs to the information retrieval system, i.e., using spoken words and not textual queries.
Moreover, due to the fact that the new paradigm employs a conversation as a mean of interaction, only one result is provided to the user as an answer to her question.
As a consequence, the precision in the identification of the only answer to return is now of paramount importance to build an effective conversational system.

State-of-the-art solutions for \revrm{performing} the task above rely on machine learning techniques~\cite{DBLP:journals/ftir/Liu09}, to select the answer with the highest relevance.
The selection of the most relevant result can be addressed in two different ways:
\textit{i}) by exploiting machine-learned techniques such as \lmart~\cite{DBLP:journals/ir/WuBSG10}, which are based on univariate scoring functions that individually estimate one candidate result at a time, to select the candidate achieving the highest relevance score;
\textit{ii}) by employing pairwise Learning-to-Rank techniques such as \dbert{} \cite{DBLP:journals/corr/abs-1901-04085}, which are based on bivariate scoring functions that estimate a pair of candidate results at a time, e.g., a binary judgment stating which of the results is more relevant, to select the candidate achieving the highest sum of pairwise scores of an all-vs-all tournament.
While the former approach exploits only the information of a single result at a time for computing the ranking score, the latter approach is potentially more powerful because it exploits the information of two candidates at a time for computing the outcome of the tournament.
However, the latter approach, although effective, is more expensive than the former one as it performs a quadratic number of comparisons to score all pairs of candidate results, thus making pairwise approaches unappealing in scenarios with tight time constraints. Here is where our research is beneficial as we define algorithmic approaches that allow reducing the number of comparisons performed to select the most relevant results thus speeding up the whole selection process.

%\lb{Esprimo il mio parere sull'intro scritta cosí. Premetto che io in genere leggo articoli solo theory, quindi non so bene come scrivere un articolo di questo genere. Negli articoli di teoria la parte di motivation é breve, e talvolta un po' pretestuale a dirla tutta... Quindi quello che si fa sempre é raccontare una breve storia sexy di perché il setting studiato merita di essere studiato e poi ci si tuffa nei dettagli tecnici della teoria. In questo caso, noi abbiamo un bel po' di piú da dire sul contesto applicativo, quindi non saprei esattamente come giocarmela. Provo comunque ad elaborare un pensiero. Il motivo per cui gli articoli di teoria vengono scritti in quel modo, da quanto ho capito, é che si vuole raccontare una storia convincente che interessi il lettore al modello /  setting studiato per incuriosirlo nei confronti della domanda (a chi interessa una domanda completamente arbitraria, in fondo?). Quello che stiamo facendo con questa introduzione é scrivere una prima pagina extra dry, e poi dare le motivazioni estensivamente. Questo va un po' contro l'idea che bisogna ``conquistarsi l'attenzione del lettore'' raccontando subito la storia sexy prima di fargli ingoiare i dettagli tecnici.}

%\lb{BOTTOM LINE: Trovo che ribaltare completamente l'esposizione renda l'intro un po' troppo difficile da digerire (molti lettori chiudono subito il pdf, prima di arrivare alle motivations). D'altro canto non rinuncerei ad una descrizione estensiva dei campi di applicazione. Penso che un giusto mezzo possa essere: (1) raccontare in breve che vogliamo usare un comparatore binario ML allo scopo di trovare l'elemento migliore, dire che il comparatore é costoso e che allo stesso tempo ci aspettiamo che sbagli poco -soprattutto quando compara l'elemento migliore-. (2) Spiegare come questo si traduce nella nostra parametrizzazione e poi tufarci a pesce nei dettagli teorici. (3) Raccontare estensivamente le applicazioni.}

\smallskip
The rest of the article is structured as follows: Section~\ref{bf:sec:related} discusses the related work, while Section~\ref{bf:sec:problem_definition} defines the problem. Section~\ref{bf:sec:complexity} provides a detailed analysis of the problem complexity and Section~\ref{bf:sec:algorithm} presents an efficient algorithm to solve it. Moreover, Section~\ref{bf:sec:generalizations} discusses two variants of that algorithm that solve two extensions of the original problem. Finally, Section~\ref{bf:sec:experiments} presents a comprehensive analysis of proposed algorithms in a information retrieval (ad-hoc search) scenario, and Section~\ref{bf:sec:summary} concludes the work.


==> sections/2.5-problem-definition.tex <==
% !TEX root = ../paper.tex
% !TeX spellcheck = en_US


\section{Problem definition}
\label{bf:sec:problem_definition}
\revchange{
We map the problem of efficiently retrieving the top-$1$ result from a list of item to the
task of finding a champion of the round-robin tournament.
A tournament $T = (V, E)$ can be modeled as a complete directed graph.
}{
A round-robin tournament between $n$ players can be modeled as a complete directed graph $T = (V, E)$.
}
Given $u, v \in V$, we say that $u$ \emph{wins} against $v$ if $(u, v) \in E$.
In several real-world applications, the direction of the arc is inferred by employing machine learning classifiers that estimate whether $u$ wins against $v$ or viceversa.
\revchange{
In the following, we call ``arc lookup'' the above estimation done on a pair of vertices, i.e., $(u,v)$.
}{
In the following, we call ``arc lookup'' or ``arc unfold'' the operation of looking at the direction of an arc between two nodes.
}
%When such a model is available, its application allows to infer the set $E$ of edges of the tournament graph $T$.

%We address the efficiency issues of the top-$1$ retrieval task when employing pairwise machine learning classifiers.
\revchange{
We define the champion as the player, i.e., one vertex of the tournament graph $T$, winning the highest number of matches in the inferred tournament graph, i.e., the Copeland winner, and our
}{
The champion of a tournament, also known as Copeland winner, is a player of the tournament winning the highest number of matches, i.e., a vertex in $V$ with the highest out-degree of the tournament graph $T$.
Our
}
goal is to find it by employing the minimum number of comparison queries, i.e., arc lookups.

If the tournament is transitive---whenever $u$ wins against $v$ and $v$ wins against $w$, then $u$ wins against $w$---we can trivially identify the unique champion with $\Theta(n)$ arc lookups.
Indeed, the champion is the only vertex that wins all its matches and, thus, we can perform a \textit{knock-out tournament} where the loser of any match is immediately eliminated.
However, finding the champion of general tournament graphs requires $\Omega(n^2)$ arc lookups~\cite{DBLP:journals/corr/GutinMR18}. As a consequence, there is nothing better to do than playing all the matches in order to find the champion. This means that the structure of the underlying tournament graph heavily impacts the complexity of the problem.

We consider therefore a novel parameterization and we define $\ell$ as the number of matches lost by the champion.
Then, we design a deterministic algorithm that solves the problem in $\Theta(\ell n)$ comparison queries
and time.
This parameterization is motivated by the fact that it is possible to design very accurate machine learning classifiers for several tasks.
For this reason, we expect a low number of matches $\ell$ lost by the most relevant item, hence a quasi-linear number of arc lookups is required by our algorithm to find it.
This compares with the quadratic number of lookups of the previously known algorithms~\cite{DBLP:journals/corr/GutinMR18}.

We first prove that $\Omega(\ell n)$ arc lookups are required to solve the problem with any deterministic algorithm.
We also prove that the same bound holds if we allow the algorithm to
be incorrect with any fixed probability.
Then, we present an asymptotically optimal deterministic algorithm to solve the problem whose time complexity matches the lower bound without any prior knowledge about the parameter $\ell$.
We finally detail how to extend our algorithm to solve interesting generalizations of the problem.
The first one asks for reporting the top-$k$ players with the highest number of wins.
Our novel algorithm solves this problem with $\Theta(n\ell_k)$ arc lookups, where $\ell_k$ is the number of matches lost by the $k$-th player.
We also present a variant of our algorithm to take full advantage of parallel inference mechanisms to perform arc lookups with a machine learning classifier, i.e., where a batch $B$ of pairwise comparisons are performed in parallel.
This is useful in practice because pairwise comparisons are batched when the inference is done on novel computing platforms like, for example, GPGPUs. \rt{Franco, si tratta di un typo??}
We show that our algorithm finds the winner by performing $O(\frac{\ell n}{B} + \ell \log B)$ arc lookups.
Finally, we generalize the tournament problem in a probabilistic framework, where each arc $(u, v) \in E$ is labeled with the likelihood that $u$ wins against $v$.
These probabilities can be interpreted as the confidence of the classifier about the outcome of the comparison.
In this framework, the goal is to find the player with the largest sum of probabilities.
To this end, we present a deterministic algorithm to find the champion of a probabilistic tournament by performing the minimum number of arc lookups needed to solve this problem.


==> tables/table1.tex <==
% !TEX root = ../paper.tex

{
\setlength{\extrarowheight}{0.15em}
\setlength{\tabcolsep}{0.8em}
\begin{tabular}{lrrr@{}l}

\toprule

Method & Recall@1 & Inferences & \multicolumn{2}{c}{Time (s)} \\

\midrule

BM25 + monoBERT
& 0.251 & 1000 & 65.91 & \\

\midrule

+ duoBERT\textsubscript{BINARY}
& 0.269 & 870 & 57.34 & \\

+ duoBERT\textsubscript{BINARY} \& Alg. \ref{bf:alg:pseudocode}
& 0.269 & 65 & 4.26 & \hspace{0.2em}\tspeedup{13.5} \\

%\midrule

%+ duoBERT\textsubscript{PROBABILISTIC}
%& 0.266 & 870 & 57.34 & \\

%+ duoBERT\textsubscript{PROBABILISTIC} \& Alg. \ref{bf:alg:pseudocode}
%& 0.266 & 179 & 8.86 & \hspace{0.2em}\tspeedup{6.5} \\

\bottomrule

\end{tabular}
}
